PDE-NetGen 1.0: from symbolic PDE representations of physical processes to trainable neural network representations

Bridging physics and deep learning is a topical challenge. While deep learning frameworks open avenues in physical science, the design of physically-consistent deep neural network architectures is an open issue. In the spirit of physics-informed NNs, PDE-NetGen package provides new means to automatically translate physical equations, given as PDEs, into neural network architectures. PDE-NetGen combines symbolic calculus and a neural network generator. The later exploits NN-based implementations of PDE solvers using Keras. With some knowledge of a problem, PDE-NetGen is a plug-and-play tool to generate physics-informed NN architectures. They provide computationally-efficient yet compact representations to address a variety of issues, including among others adjoint derivation, model calibration, forecasting, data assimilation as well as uncertainty quantification. As an illustration, the workflow is first presented for the 2D diffusion equation, then applied to the data-driven and physics-informed identification of uncertainty dynamics for the Burgers equation.

==> makefile <==
# Liste des .pdf du projet
PDF=arxiv-main.pdf

# Variable d'environnement 
REP=$(shell pwd | awk -F / '{print $$NF }')

# Commande de compilation
LATEX = pdflatex -interaction=batchmode
#LATEX = pdflatex 
BIBTEX = bibtex -terse
JABREF = java -jar /usr/share/jabref/jabref
#BIBTEX = bibtex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
UNDEFINED = "((Reference|Citation).*undefined)|(Label.*multiply defined)"
	#Dépendance pour les .pdf
TEX=$(PDF: .pdf = .tex)

#
#	Commande de compilation
#
pdffiles: $(PDF)

# Commande de compilation
%.pdf : %.tex
	@echo "Compilation du tex"
	@$(LATEX) $<
	# OLD: If file `database.bib` is present then extract bibliography from it
	# 
	#  If citation needs to be update, then `make subdatabase`
	#
ifeq ("$(wildcard database.bib)","database.bib")
	#@$(JABREF) -a $*,$*_database database.bib -n > jabref.log
endif
	#@makeindex $*
	@# Etape de compilation suivant la nécessité.
	@if egrep -q $(RERUN) $*.log ; then echo "passe BibTex/LaTeX" ;\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@if egrep -q $(RERUN) $*.log ; then echo "passe BibTex/LaTeX" ;\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@if egrep -q $(UNDEFINED) $*.log ; then echo "passe Complémentaire";\
	$(BIBTEX) $* ; $(LATEX) $<;  fi
	@# Vérification de la présence de toute la biblio.
	@egrep -i $(UNDEFINED) $*.log || echo "Dépendance biblio non manquante"
	@exit 0

save:
	make clean
	cd .. ; tar --dereference -cvzf $(REP).tgz $(REP) ; horodate $(REP).tgz
clean:
	rm -f *.dvi *.ps *.log *.aux *.out  *.idx *.toc *.blg *.bbl \
		*.ind *.ilg *.nav *.snm
	#rm -f *_database.bib *_database.bib.bak
	rm -f `find | grep .*~`
cleanall: clean
	rm -f *.pdf
header:
	ln -sf ~/work/newdoc/latex/header.tex
	ln -sf ~/work/newdoc/latex/header-private.sty
	ln -sf ~/work/newdoc/latex/header-pres.tex
	ln -sf ~/work/newdoc/latex/set_demo
	ln -sf ~/pdf/database.bib
install:
	cp -f ~/work/newdoc/latex/ametsoc.* .
	cp -f ~/work/newdoc/latex/widetext.sty .
	cp -f ~/work/newdoc/latex/beamer* .
	cp -rf ~/work/newdoc/latex/logo .
	cp -i ~/work/newdoc/latex/paper.tex .
	cp -i ~/work/newdoc/latex/pres.tex .
	cp -i ~/work/newdoc/latex/poster.tex .
	cp -f ~/work/newdoc/latex/.gitignore .
	make header
	mkdir figures
	mkdir src
	mkdir version
update:
	cp -f ~/work/newdoc/latex/makefile .

subdatabase:
	@echo "Create a database from the .aux file"
	@$(JABREF) -a main,main_database database.bib -n > jabref.log


#
#  Export in asimpler form
#
EXPORT_DIR = ./tmp/export_paper/

export:
	mkdir -p $(EXPORT_DIR)
	cp ./paper.tex ./makefile ./widetext.sty  \
		./paper_database.bib ./ametsoc.bst $(EXPORT_DIR)
	# Don't load figures for export.
	./set_demo ./header-private.sty $(EXPORT_DIR)header-private.sty
	

#
#  Construct difference file and prepare compilation for editting
#

DIFF_DIR = ./diff/
VERSION_OF_REFERENCE = ./version/main.tex

paper_diff:
	# 1. Create directory for diff.
	mkdir -p $(DIFF_DIR)
	# 2. Copy local files for the compilation
	cp ./makefile ./widetext.sty  \
		./main_database.bib ./ametsoc.bst $(DIFF_DIR)
	cp -rf ./figures/ $(DIFF_DIR)
	# 3. Don't load figures for export.
	#./set_demo ./header-private.sty $(DIFF_DIR)header-private.sty
	# 4. Create the `diff file` 
	latexdiff $(VERSION_OF_REFERENCE) ./main.tex > $(DIFF_DIR)main.tex
	

